Blinding scheme for the scale-dependence bias signature of local primordial non-Gaussianity for DESI 2024

The next generation of spectroscopic surveys is expected to achieve an unprecedented level of accuracy in the measurement of cosmological parameters. To avoid confirmation bias and thereby improve the reliability of these results, blinding procedures become a standard practice in the cosmological analyses of such surveys. Blinding is especially crucial when the impact of observational systematics is important relative to the cosmological signal, and a detection of that signal would have significant implications. This is the case for local primordial non-gaussianity, as probed by the scale-dependent bias of the galaxy power spectrum at large scales that are heavily sensitive to the dependence of the target selection on the imaging quality, known as imaging systematics. We propose a blinding method for the scale-dependent bias signature of local primordial non-gaussianity at the density field level which consists in generating a set of weights for the data that replicate the scale-dependent bias. The applied blinding is predictable, and can be straightforwardly combined with other catalog-level blinding procedures that have been designed for the baryon acoustic oscillation and redshift space distortion signals. The procedure is validated through simulations that replicate data from the first year of observation of the Dark Energy Spectroscopic Instrument, but may find applications to other upcoming spectroscopic surveys.

==> contents/note.tex <==
\clearpage
\newpage

\section{Maths}

Using the ergodicity $<w_{blind}> = <w_{blind}>_{\vb{x}}$. the multiplication in Fourier is the convolution in real space such that
\begin{align}
<w_{blind}(\vb{x})> &= <w_{blind}>_{\vb{x}} \\
    &= \dfrac{1}{V} \int \dd{\vb{x}} (a \star \delta^r) \\
    &=  \dfrac{1}{V} \int \dd{\vb{x}} \int \dd{\vb{y}}a(\vb{y}) \times \delta^r(\vb{x}-\vb{y}) \\
    &=  \dfrac{1}{V} \int \dd{\vb{y}} a(\vb{y}) \int \dd{\vb{x}} \delta^r(\vb{x}-\vb{y}) \\
    &=  0,
\end{align}
since $\int \dd{\vb{x}} \delta^r(\vb{x}-\vb{y}) = <\delta^r>_{\vb{x}} = 0$.

\section{First version}

We note that the grid we use have a cell size half smaller than the smoothing radius, such that smoothing due to painting / reading steps is neglected.

such that the estimated density field on the grid is in Fourier space: 
\begin{equation}
   \widehat{\delta}(\vb{k}) = W^{\mathrm{cic}}(\vb{k}) \delta(\vb{k})
\end{equation}
where
\begin{equation}
W^{\mathrm{cic}}(\vb{k}) = W^{\mathrm{cic}}(k_x)W^{\mathrm{cic}}(k_y) W^{\mathrm{cic}}(k_z) \quad \text{with} \quad
W^{\mathrm{cic}}(k) = \mathrm{sinc}^2\left(\dfrac{\pi k}{2 k_N} \right)
\end{equation}
and $k_N = \pi / H$ is the Nyquist frequency corresponding to the grid cell size $H$.
where $$W^{\mathrm{cic}}(k) = \mathrm{sinc}^2\left(\dfrac{\pi k}{2 k_N} \right)$$ with $k_N = \pi / H$ the Nyquist frequency corresponding to the cell size $H$. Here, we assume the window function to be \textit{isotropic}, as an approximation for the 3D: $$W^{\mathrm{cic}}(\vb{k}) = W^{\mathrm{cic}}(k_x)W^{\mathrm{cic}}(k_y) W^{\mathrm{cic}}(k_z).$$

Since we only need to reconstruct the real-space density field at large scales (where PNG matters), the density field is additionally smoothed by the isotropic Gaussian kernel function 
\begin{equation}
   W^s(\vb{k}) = \exp(-\frac{1}{2}k^2\sigma^2),
\end{equation}
where $\sigma = 30~h^{-1}\textrm{Mpc}$ is the smoothing radius. This kernel is displayed in \cref{fig:window_reconstrucion} for several values of $\sigma$. The larger the smoothing parameter, the more the fluctuations of the reconstructed density field on small scales (large $k$) will be suppressed. The smoothing parameter allows us to control which scales will be affected by this blinding scheme, thereby preventing the BAO or RSD scales from being contaminated by these additional weights. More details on the effect of smoothing will be given in \cref{sec:lower_bias}.

Finally, $w_{\phantom{d}\mathrm{blind}}^{d}(\vb{x})$ is read from the FFT of $a(k) \times \widehat{\delta}^r(\vb{k})$ with the CIC scheme at the galaxy positions.


, leading to an additional $W^{\mathrm{cic}}(k)$ contribution. Hence, the total window function, which is applied to the density field, reads as
\begin{equation}
W^{\mathrm{tot}}(k) = W^s(k) \times W^{\mathrm{cic}}(k)^2,
\end{equation}
and the reconstructed field that we evaluate is such that
\begin{equation} %\label{eqn:window}
\langle \vert \widehat{\delta}^r(k) \vert^2 \rangle \propto W^{\mathrm{tot}}(k)^2 \times \left[b^2P_{\mathrm{lin}}(k) + 1/n\right],
\end{equation}
where $1/n$ is an undesired shot noise term. As described in \cref{sec:shotnoise_correction}, not correcting it will bias the blinding procedure.

%For the same reason as the window $W^{\mathrm{tot}}(k)$ appears in \cref{eqn:window}, the displacement field $\psi$ is also computed from the smoothed density field (with only one cic-reading) and $\sigma_d$ must be re-scaled as
%\begin{equation}
%    \sigma_d^2 = \frac{1}{6\pi} \int \dd k (W^s W^{\mathrm{cic}})^{2}(k) P_{\mathrm{lin}}(k).
%\end{equation}


\section{OLD STUFF}

Some brief remarks on the above equations \cref{eqn:power_spectrum_with_blinding_weights}:
\begin{itemize}
    \item The shot-noise can be supposed similar between the redshift space distribution and the real space distribution since the size of fluctuations of $n(x)$ are much smaller than the displacement field.
    \item 
    This can be achieved easily: 
    \begin{lstlisting} 
        pk_lin.clone(k=pk_lin, pk=W(k)**2 * % pk_lin(k)).sigma_d()**2 
    \end{lstlisting}
\end{itemize}



\subsection{Double blinding}

\red{Evidement pas une tres bonne idee vu la tete de W(k) ...} In order to remove this undesired effect, the proposed weights are modified as
\begin{equation}
a(k) \longrightarrow a(k) \equiv \dfrac{a(k)}{W(k)}.
\end{equation}
\red{avec ton faire avec .. on peut pas faire autrement de toute facon et on va le mettre dans le poids. le mettre en remarque pour dure que ce n'etait pas une bonne idee...}

\textbf{Note:} $\langle \psi_u \delta_m \rangle = 0$ since $\int dk^3 \hat{k} P(k) = \int k^2 P(k) dk \underbrace{\int_{sphere} \hat{k}}_{=0}$.

pour comprendre l'estimateur apres la reconstruction : \citep{Taruya2010}

\textbf{remarque:} Il y a biensur une window function pour une boite cubic lorsque los n'est pas un axe de laboite, c'est plus périodique! attention, dans notre cas on a deplacé les particules selon z .. ca va avoir un impact ? essayer !

Attention, il y a quoi qu'il arrive une windonw fonction (boite ou cutsky) due au subsampling sur la grille tout simplement, comme pour la reconstruction. On suppose, légitimement, que cette window est néglegeable .. (ie) qu'on est loin de la fréquence de Nyquist.

